Average-Case Hardness of Binary-Encoded Clique in Proof and Communication Complexity

We study the average-case hardness of establishing that a graph does not have a large clique in both proof and communication complexity. We show exponential lower bounds on the length of cutting planes and bounded-depth resolution over parities refutations of the binary encoding of clique formulas on randomly sampled dense graphs. Moreover, we show that the randomized communication complexity of finding a falsified clause in these formulas is polynomial.

==> restate.tex <==
\usepackage{thmtools,thm-restate}
\theoremstyle{plain}
\declaretheorem[sibling=theorem,name=Theorem]{restatabletheorem}
\declaretheorem[sibling=theorem,name=Lemma]{restatablelemma}

\makeatletter
\renewenvironment{thmt@restatable}[3][]{%
  \thmt@toks{}% 
  \stepcounter{thmt@dummyctr}% 
  \long\def\thmrst@store##1{%
    \@xa\gdef\csname #3\endcsname{%
      \@ifstar{%
        \thmt@thisistheonefalse\csname thmt@stored@#3\endcsname
      }{%
        \thmt@thisistheonetrue\csname thmt@stored@#3\endcsname
      }%
    }%
    \@xa\long\@xa\gdef\csname thmt@stored@#3\@xa\endcsname\@xa{%
      \begingroup
      \ifthmt@thisistheone
        % 
      \else
        \@xa\protected@edef\csname the#2\endcsname{%
          \thmt@trivialref{thmt@@#3}{??} (Restated)}%
        %
        \ifcsname r@thmt@@#3\endcsname\else
          \G@refundefinedtrue
        \fi
        % 
        \@xa\let\csname c@#2\endcsname=\c@thmt@dummyctr
        \@xa\let\csname theH#2\endcsname=\theHthmt@dummyctr
        % 
        \let\label=\@gobble
        \let\ltx@label=\@gobble% 
        % 
        \def\thmt@restorecounters{}%
        \@for\thmt@ctr:=\thmt@innercounters\do{%
          \protected@edef\thmt@restorecounters{%
            \thmt@restorecounters
            \protect\setcounter{\thmt@ctr}{\arabic{\thmt@ctr}}%
          }%
        }%
        % 
        \thmt@trivialref{thmt@@#3@data}{}%
      \fi
      % 
      \ifthmt@restatethis
        \thmt@restatethisfalse
      \else
        \csname #2\@xa\endcsname\ifx\@nx#1\@nx\else[{#1}]\fi
      \fi
      \ifthmt@thisistheone
         % 
         \thmt@rst@storecounters{#3}%
        % 
        \label{thmt@@#3}%
      \fi
      % 
      ##1%
      \csname end#2\endcsname
      % 
      \ifthmt@thisistheone\else\thmt@restorecounters\fi
      \endgroup
    }% 
    \csname #3\@xa\endcsname\ifthmt@thisistheone\else*\fi
    %
    \@xa\end\@xa{\@currenvir}
  }%
  \thmt@collect@body\thmrst@store
}{%
  %% 
}
\makeatother

